Maximum Mean Discrepancy Distributionally Robust Nonlinear Chance-Constrained Optimization with Finite-Sample Guarantee

This paper is motivated by addressing open questions in distributionally robust chance-constrained programs (DRCCP) using the popular Wasserstein ambiguity sets. Specifically, the computational techniques for those programs typically place restrictive assumptions on the constraint functions and the size of the Wasserstein ambiguity sets is often set using costly cross-validation (CV) procedures or conservative measure concentration bounds. In contrast, we propose a practical DRCCP algorithm using kernel maximum mean discrepancy (MMD) ambiguity sets, which we term MMD-DRCCP, to treat general nonlinear constraints without using ad-hoc reformulation techniques. MMD-DRCCP can handle general nonlinear and non-convex constraints with a proven finite-sample constraint satisfaction guarantee of a dimension-independent $\mathcal{O}(\frac{1}{\sqrt{N}})$ rate, achievable by a practical algorithm. We further propose an efficient bootstrap scheme for constructing sharp MMD ambiguity sets in practice without resorting to CV. Our algorithm is validated numerically on a portfolio optimization problem and a tube-based distributionally robust model predictive control problem with non-convex constraints.

==> chapters/future_work.tex <==
This section is for the cut-out materials for future works.

{\color{red}
JZ: Todo:
\begin{itemize}
    % \item plug in the concrete tail and rates
    \item possible to bound the $\sup$-risk by Characterizing the sub-optimality of the "objective"
    \item give some examples of the first rate for nonlinear classes, NN, kernel, high order polyn, etc.
\end{itemize}
}

where $\F:=\fclass$ denotes the class of functions in the constraint of interest.
The Radmacher complexity of a function class is denoted using $\R (\cdot)$.
\jz{double check:}
Furthermore, the $\oneOverRootN$ term does not depend on dimensions.


\subsection{Refined analysis beyond the $\oneOverRootN$ rate}
In the finite-sample guarantee above, we used the global version of the Radmacher complexity, i.e., we considered the the complexity of the whole function class.
We now show, through standard refined analysis using localization~\cite{bartlettLocalRademacherComplexities2005}, we can improve on the conservative $\oneOverRootN$.
\begin{proposition}
    [Refined guarantee for \mmdsp{}]
    Under the same assumptions of Proposition~\ref{thm:guarantee}.
% \begin{equation}
%     \begin{aligned}
        \begin{multline}
            \pzCVaR_{1-\alpha}[f(\xh, \xi)] \leq\\
            \frac{6K}{B}(\R(\fclassLocal)+\rhatstar)\\
            + \oneOverN.
        \end{multline}
%     \end{aligned}
% \end{equation}
where $\rhatstar \leq ...$.
% where $\E\to 0$ as $n\to\infty$.
\end{proposition}

\begin{proof}
    The proof is similar but uses the local analysis \cite[Theorem~4.1]{bartlettLocalRademacherComplexities2005}.
    For any $K>1$,
    % \begin{multline}
        \begin{equation*}
            \begin{aligned}
            \Etrue( [f(x,\xi) + t]_+ - \gh )\\
            \leq
            \frac{K}{K-1}
            \Ehat( [f(x,\xi) + t]_+ - \gh )
            \\
            +\frac{6K}{B}(\R(\fclassLocal)+\rhatstar)\\
             + \oneOverN
            .
        \end{aligned}
    \end{equation*}
    % \end{multline}
    where $\rhatstar \leq ...$
    {
        \color{red}
        JZ:
        \begin{itemize}
            \item explain what B is; bound the var of f
            \item also cite the refined analysis in \cite{namkoongVariancebasedRegularizationConvex}
        \end{itemize}
        }
\end{proof}
In the case that empricial kernel Gram matrices have exponential decay eigenvalues, as satisfied by common kernels such as the Gaussian kernel, the rate above can be as fast as $\logNOverN$.
Furthermore, if there are only finitely-many non-zero eigenvalues, the decay can be as fast as $\oneOverN$.
\begin{remark}
    We note that this is no "free lunch" since we will still be limited by the local complexity of the class $\fclass$.
    Nonetheless, our analysis here already greatly generalizes over the analysis in the Wasserstein ambiguity set approaches.
\end{remark}

\jz{from feasibility to optimality, discuss rate vs eq 7}{}

